Overview of the TREC 2021 Fair Ranking Track

The TREC Fair Ranking Track aims to provide a platform for participants to develop and evaluate novel retrieval algorithms that can provide a fair exposure to a mixture of demographics or attributes, such as ethnicity, that are represented by relevant documents in response to a search query. For example, particular demographics or attributes can be represented by the documents' topical content or authors. The 2021 Fair Ranking Track adopted a resource allocation task. The task focused on supporting Wikipedia editors who are looking to improve the encyclopedia's coverage of topics under the purview of a WikiProject. WikiProject coordinators and/or Wikipedia editors search for Wikipedia documents that are in need of editing to improve the quality of the article. The 2021 Fair Ranking track aimed to ensure that documents that are about, or somehow represent, certain protected characteristics receive a fair exposure to the Wikipedia editors, so that the documents have an fair opportunity of being improved and, therefore, be well-represented in Wikipedia. The under-representation of particular protected characteristics in Wikipedia can result in systematic biases that can have a negative human, social, and economic impact, particularly for disadvantaged or protected societal groups.

==> participants.tex <==
\section{Potential Participants}

We expect continued interest from the community that has already formed around the problem of fairness in information retrieval and recommendation.
This includes participants from past TRECs, the FAcccTrec Workshop on Responsible Recommendation, and the FACTS-IR workshop at SIGIR.
We are also hoping this year to recruit additional groups through targeted outreach to members of the Fairness, Accountability, and Transparency (FAccT) community, capitalizing on existing interest in the topic.


==> submitting.tex <==
\section{Submission Instructions}

TBA with eval data.
